Metric-like spaces as enriched categories: three vignettes

This is a write-up of a talk given at the CATMI meeting in Bergen in July 2023, and is an introduction to a category-theoretic perspective on metric spaces. A metric space is a set of points such that between each pair of points there is a number -- the distance -- such that the triangle inequality is satisfied; a small category is a set of objects such that between each pair of objects there is a set -- the hom-set -- such that elements of the hom-sets can be composed. The analogy between the structures that can be made in to a common generalization of the two structures, so that both are examples of enriched categories. This gives a bridge between category theory and metric space theory. I will describe this and three examples from around mathematics where this perspective has been useful or interesting. The examples are related to the tight span, the magnitude and the Legendre-Fenchel transform.

==> figs/fig2pstex <==
#! /bin/zsh -f
for fig in *.fig; do
  if [[ -e ../pstex/${fig:r}.eps && ../pstex/${fig:r}.eps -nt $fig ]]; then
	print "Skipping   ${fig:r}"
   else
        print "Processing ${fig:r}"
	print ${fig:r}
	fig2dev -L pstex  $fig ../pstex/${fig:r}.eps
	epstopdf ../pstex/${fig:r}.eps -o ../pstex/${fig:r}.pdf
	fig2dev -L pstex_t -F -p "\\figdir/${fig:r}" $fig ../pstex/${fig:r}.pstex_t
 fi
done


